Unbiased Spectroscopic Study of the Cygnus Loop with LAMOST. I. Optical Properties of Emission Lines and the Global Spectrum

We present an unbiased spectroscopic study of the Galactic supernova remnant (SNR) Cygnus Loop using the Large Sky Area Multi-object Fiber Spectroscopic Telescope (LAMOST) DR5. LAMOST features both a large field of view and a large aperture, which allow us to simultaneously obtain 4000 spectra at $\sim$3700-9000 \AA with R$\approx$1800. The Cygnus Loop is a prototype of middle-aged SNRs, which has the advantages of being bright, large in angular size, and relatively unobscured by dust. Along the line of sight to the Cygnus Loop, 2747 LAMOST DR5 spectra are found in total, which are spatially distributed over the entire remnant. This spectral sample is free of the selection bias of most previous studies, which often focus on bright filaments or regions bright in [O III]. Visual inspection verifies that 368 spectra (13$\%$ of the total) show clear spectral features to confirm their association with the remnant. In addition, 176 spectra with line emission show ambiguity of their origin but have a possible association to the SNR. In particular, the 154 spectra dominated by the SNR emission are further analyzed by identifying emission lines and measuring their intensities. We examine distributions of physical properties such as electron density and temperature, which vary significantly inside the remnant, using theoretical models. By combining a large number of the LAMOST spectra, a global spectrum representing the Cygnus Loop is constructed, which presents characteristics of radiative shocks. Finally, we discuss the effect of the unbiased spectral sample on the global spectrum and its implication to understand a spatially unresolved SNR in a distant galaxy.

==> tabA1.tex <==


%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Wed Nov  7 00:54:49 2018

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.
%%\documentclass{aastex}
%%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.
\begin{deluxetable}{ccc}\label{tab:A1}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{Table A1.}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment 
%% all other tables after this table based on this number
%\tablenum{A1}

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the 
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the 
%% correct number of &s.
\tablehead{\colhead{Obs. ID} & \colhead{R.A.} & \colhead{Decl.} \\ 
\colhead{} & \colhead{(2000)} & \colhead{(2000)} } 

%% All data must appear between the \startdata and \enddata commands
\startdata
%  Line ID &  R.A. &  Dec \\
 470503073 &  20:48:14.25 &  29:48:18.2 \\
 470503103 &  20:47:08.01 &  30:12:42.0 \\
 470503109 &  20:46:57.83 &  30:01:30.0 \\
 470503144 &  20:50:34.10 &  30:09:36.4 \\
 470503149 &  20:50:25.41 &  30:07:23.3 \\
 470503216 &  20:48:55.01 &  30:14:17.8 \\
 470504035 &  20:52:49.22 &  29:55:58.8 \\
 470504061 &  20:52:46.06 &  29:21:47.8 \\
 470504132 &  20:51:38.97 &  29:13:15.0 \\
 470504139 &  20:52:06.30 &  29:10:53.2 \\
 470504144 &  20:51:53.28 &  29:11:51.1 \\
 470504151 &  20:50:35.79 &  29:47:10.4 \\
 470505053 &  20:51:16.10 &  28:48:00.5 \\
 470509027 &  20:56:20.14 &  30:23:39.4 \\
 470509075 &  20:56:45.43 &  30:54:45.8 \\
 470509080 &  20:56:05.12 &  31:05:26.6 \\
 470509089 &  20:56:38.60 &  31:05:17.8 \\
 470509097 &  20:56:16.90 &  31:04:53.9 \\
 470509098 &  20:57:10.59 &  30:58:13.3 \\
 470511036 &  20:55:45.44 &  31:48:16.2 \\
 470511039 &  20:55:32.11 &  31:47:40.1 \\
 470511109 &  20:56:03.14 &  31:41:23.8 \\
 470511160 &  20:50:26.14 &  32:03:16.8 \\
 470511161 &  20:51:15.44 &  31:53:00.4 \\
 470511167 &  20:50:46.95 &  32:00:25.2 \\
 470511185 &  20:52:40.27 &  31:43:32.9 \\
 470511201 &  20:54:14.04 &  31:58:15.0 \\
 470511223 &  20:54:06.80 &  32:08:03.9 \\
 470512067 &  20:57:08.80 &  31:19:39.5 \\
 470512069 &  20:57:14.69 &  31:23:38.4 \\
 470512080 &  20:57:06.17 &  31:13:51.6 \\
 470512083 &  20:57:20.03 &  31:04:17.3 \\
 470512084 &  20:56:53.09 &  31:07:44.5 \\
 470512087 &  20:57:15.97 &  31:14:52.0 \\
 470512129 &  20:57:03.88 &  31:10:49.2 \\
 470512135 &  20:56:09.67 &  31:14:37.3 \\
 470512137 &  20:56:10.23 &  31:09:33.9 \\
 470512241 &  20:56:40.97 &  31:43:42.7 \\
 470514093 &  20:46:04.69 &  30:27:51.6 \\
 470514094 &  20:46:02.87 &  30:35:40.6 \\
 470514096 &  20:46:39.28 &  30:19:23.1 \\
 470514141 &  20:45:28.02 &  30:35:53.1 \\
 470514142 &  20:45:50.21 &  30:40:34.4 \\
 470514165 &  20:46:22.67 &  30:15:00.3 \\
 470514168 &  20:46:18.01 &  30:21:37.6 \\
 470515006 &  20:52:15.39 &  30:52:44.2 \\
 470515065 &  20:48:26.39 &  30:35:39.6 \\
 470515199 &  20:51:46.06 &  30:20:22.4 \\
 470516089 &  20:46:04.54 &  30:54:49.2 \\
 470516108 &  20:50:16.41 &  31:15:16.6 \\
 470516172 &  20:48:42.47 &  31:05:55.1 \\
 470516174 &  20:48:55.01 &  31:13:30.6 \\
 470516184 &  20:47:02.23 &  30:57:17.1 \\
 470516229 &  20:48:03.32 &  31:40:31.5 \\
 470516246 &  20:48:47.85 &  31:53:14.9 \\
 475203151 &  20:48:15.30 &  29:46:09.1 \\
 475211039 &  20:55:30.57 &  31:50:28.3 \\
 475211106 &  20:55:19.13 &  31:51:01.9 \\
 475211136 &  20:52:43.27 &  31:55:29.0 \\
 475211152 &  20:51:00.47 &  31:51:28.3 \\
 475211160 &  20:50:39.07 &  32:04:39.3 \\
 475211213 &  20:53:37.24 &  32:06:04.0 \\
 475212060 &  20:56:23.61 &  31:35:05.4 \\
 475212080 &  20:57:08.79 &  31:14:17.0 \\
 475212129 &  20:56:48.79 &  31:12:41.9 \\
 475212236 &  20:56:36.43 &  31:40:08.9 \\
 475214088 &  20:46:06.49 &  30:22:10.5 \\
 475214135 &  20:46:08.99 &  30:43:46.9 \\
 475215159 &  20:49:16.88 &  30:53:37.8 \\
 475215190 &  20:51:43.39 &  30:23:35.9 \\
 475216143 &  20:48:45.24 &  31:29:15.5 \\
 475216147 &  20:48:42.52 &  31:36:13.9 \\
 475216228 &  20:48:20.02 &  31:44:40.4 \\
 475216229 &  20:48:13.46 &  31:41:44.1 \\
 475216241 &  20:48:23.97 &  31:55:56.5 \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and 
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable}


